SeGuE: Semantic Guided Exploration for Mobile Robots

The rise of embodied AI applications has enabled robots to perform complex tasks which require a sophisticated understanding of their environment. To enable successful robot operation in such settings, maps must be constructed so that they include semantic information, in addition to geometric information. In this paper, we address the novel problem of semantic exploration, whereby a mobile robot must autonomously explore an environment to fully map both its structure and the semantic appearance of features. We develop a method based on next-best-view exploration, where potential poses are scored based on the semantic features visible from that pose. We explore two alternative methods for sampling potential views and demonstrate the effectiveness of our framework in both simulation and physical experiments. Automatic creation of high-quality semantic maps can enable robots to better understand and interact with their environments and enable future embodied AI applications to be more easily deployed.

==> figures/bytes_map_visualization.tex <==
\begin{figure}[!t]
%\vspace{6pt}
    \centering
    \subfloat[SeGuE Occupancy]{\includegraphics[width=0.13\textwidth,trim={155 11 161 45},clip]{images/Bytes/occupancy.pdf}}%
    \hspace{0.01\textwidth}
    \subfloat[SeGuE Semantics]{\includegraphics[width=0.13\textwidth,trim={37 10 71 55},clip]{images/Bytes/semantic_cls_no_label.pdf}}%
    \caption{Mapping results of SeGuE in real-world experiments.}
    \label{fig:bytes_map_visualization}
\end{figure}

==> sections/6_limitations.tex <==
\section{Limitations}
Our proposed method builds off the well-known next-best-view algorithm to perform semantic exploration. It will have all the same limitations and drawbacks associated with next-best-view methods, particularly the performance dependence on the sampling method and scoring. In particular, our scoring method considers only the information gain of a particular pose, ignoring that much of the information gain happens during navigation between poses. Additionally, we focused only on global sampling methods to avoid getting trapped in local minima. This leads to inefficient motion when poses on opposite sides of the map are chosen. The trade-offs between global and local sampling have been previously studied in \cite{selin2019efficient} and could be adapted to our method as a future work. 

==> tables/bytes_metrics.tex <==
\begin{table}[t]
    \centering
    \caption{Real-World Results}
        \begin{tabular}{ccc}
            \toprule
            & Coverage & Average Entropy\\
            \midrule
            & $0.735$ & $1.753$\\
            \bottomrule
        \end{tabular}
    \label{tab:real_world_results}
\end{table}
